Avalanches in the Raise and Peel model in the presence of a wall

We investigate a non-equilibrium one-dimensional model known as the raise and peel model describing a growing surface which grows locally and has non-local desorption. For specific values of adsorption ($u_a$) and desorption($u_d$) rates the model shows interesting features. At $u_a = u_d$, the model is described by a conformal field theory (with conformal charge $c=0$) and its stationary probability canbe mapped to the ground state of the XXZ quantum chain. Moreover, for $u_a \geq u_d$, the model shows a phase in which the the avalanche distribution is scale invariant. In this work we study the surface dynamics by looking at avalanche distributions using Finite-size Scaling formalism and explore the effect of adding a wall to the model. The model shows the same universality for the cases with and without a wall for an odd number of tiles removed, but we find a new exponent in the presence of a wall for an even number of avalanches released. We provide new conjecture for the probability distribution of avalanches with a wall obtained by using exact diagonalization of small lattices and Monte-Carlo simulations.

==> FIGS/e135.tex <==
\par\vspace{10mm}
$
 \put(160,55){\oval(80,50)[b]} 
 \put(160,0){\oval(80,50)[t]} 
 \put(40.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(-40.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(120.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(200.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(280.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(360.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(-50,-20){\tiny{1}} 
 \put(28,-20){\tiny{2}}
 \put(110,-20){\tiny{3}} 
 \put(190,-20){\tiny{4}} 
 \put(275,-20){\tiny{5}} 
 \put(355,-20){\tiny{6}} 
$  
\par\vspace{-1mm}
$
 \put(620,25){\vector(1,0){100}}
 \put(320,55){\oval(80,50)[b]} 
 \put(320,0){\oval(80,50)[t]} 
 \put(40.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(-40.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(120.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(200.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(280.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(360.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(-50,-20){\tiny{1}} 
 \put(28,-20){\tiny{2}}
 \put(110,-20){\tiny{3}} 
 \put(190,-20){\tiny{4}} 
 \put(275,-20){\tiny{5}} 
 \put(355,-20){\tiny{6}} 
 \put(1320,55){\oval(80,50)[b]} 
 \put(1320,0){\oval(80,50)[t]}
 \put(1160,55){\oval(80,50)[b]} 
 \put(1160,0){\oval(80,50)[t]}  
 \put(1000,55){\oval(80,50)[b]} 
 \put(1000,0){\oval(80,50)[t]} 
% \put(1040.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(960.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(1120.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(1200.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(1280.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(1360.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(950,-20){\tiny{1}} 
 \put(1028,-20){\tiny{2}}
 \put(1110,-20){\tiny{3}} 
 \put(1190,-20){\tiny{4}} 
 \put(1275,-20){\tiny{5}} 
 \put(1355,-20){\tiny{6}} 
$  \\
\par\vspace{-6mm}
$
 \put(0,55){\oval(80,50)[b]} 
 \put(0,0){\oval(80,50)[t]} 
% \put(40.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
% \put(-40.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(120.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(200.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(280.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(360.0,0.0){\rule[-0.200pt]{0.500pt}{12pt}}
 \put(-50,-20){\tiny{1}} 
 \put(28,-20){\tiny{2}}
 \put(110,-20){\tiny{3}} 
 \put(190,-20){\tiny{4}} 
 \put(275,-20){\tiny{5}} 
 \put(355,-20){\tiny{6}} 
$  \\



==> FIGS/rpm_symbols.tex <==
\newcommand{\rra}{${| 
\put(20,0){{\makebox(0,0){$\Diamond$}}}
\put(50,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~\rangle                                                                                                              
}$
}


\newcommand{\rrb}{${| 
\put(20,0){{\makebox(0,0){$\Diamond$}}}
\put(50,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(35,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~\rangle                                                                                                              
}$
}


\newcommand{\rrra}{${| 
\put(05,0){{\makebox(0,0){$\Diamond$}}}
\put(30,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(55,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle                                                                                                              
}$
}

\newcommand{\rrrb}{${| 
\put(05,0){{\makebox(0,0){$\Diamond$}}}
\put(30,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(55,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(17.5,22){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle                                                                                                              
}$
}

\newcommand{\rrrc}{${| 
\put(05,0){{\makebox(0,0){$\Diamond$}}}
\put(30,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(55,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(42.5,22){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle                                                                                                              
}$
}


\newcommand{\rrrd}{${| 
\put(05,0){{\makebox(0,0){$\Diamond$}}}
\put(30,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(55,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(17.5,22){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(42.5,22){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle                                                                                                              
}$
}

\newcommand{\rrre}{${|
\put(05,0){{\makebox(0,0){$\Diamond$}}}
\put(30,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(55,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(17.5,22){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(42.5,22){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(30,44){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle 
}$
}


==> FIGS/rpm_symbols_RPMW.tex <==
\newcommand{\wwwa}{${| 
\put(20,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(47.5,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle                                                                                                              
}$
}

\newcommand{\wwwb}{${| 
\put(20,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(47.5,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(04.5,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle                                                                                                              
}$
}

\newcommand{\wwwc}{${| 
\put(20,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(47.5,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(33.5,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle                                                                                                              
}$
}


\newcommand{\wwwd}{${| 
\put(20,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(47.5,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(04.5,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(33.5,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle                                                                                                              
}$
}

\newcommand{\wwwe}{${|
\put(20,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(47.5,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(04.5,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(33.5,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(20,40){{\makebox(0,0){$\Diamond$}}}                                                                                  
~~~~\rangle 
}$
}


\newcommand{\wwwf}{${|~
\put(20,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(47.5,0){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(04.5,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(33.5,20){{\makebox(0,0){$\Diamond$}}}                                                                                  
\put(20,40){{\makebox(0,0){$\Diamond$}}}
\put(4.5,65){{\makebox(0,0){$\Diamond$}}}                                                                                                                                                                    
~~~~\rangle 
}$
}


